Video Stream Retrieval of Unseen Queries using Semantic Memory

Retrieval of live, user-broadcast video streams is an under-addressed and increasingly relevant challenge. The on-line nature of the problem requires temporal evaluation and the unforeseeable scope of potential queries motivates an approach which can accommodate arbitrary search queries. To account for the breadth of possible queries, we adopt a no-example approach to query retrieval, which uses a query's semantic relatedness to pre-trained concept classifiers. To adapt to shifting video content, we propose memory pooling and memory welling methods that favor recent information over long past content. We identify two stream retrieval tasks, instantaneous retrieval at any particular time and continuous retrieval over a prolonged duration, and propose means for evaluating them. Three large scale video datasets are adapted to the challenge of stream retrieval. We report results for our search methods on the new stream retrieval tasks, as well as demonstrate their efficacy in a traditional, non-streaming video task.

==> relatedwork2.tex <==
% !TEX root =  bmvc_maxwelling.tex
\section{Related Work}

\cs{Need to introduce: briefly concept tradition in video \cite{SnoekFNTIR09}, pooling for video \cite{jiang2010trecvid,xu2015,NagelBMVC15} especially for events, zero-shot for events and actions, especially Mihir. End with observation that we can do any query.}

Our approach for live stream retrieval is inherently related to a wide gamut of related video tasks. 
This work falls broadly into three categories: video concept detection, temporal localisation, and classification without examples, which we discuss next.

\subsection{Exploiting Temporal Information}

The bulk of work on video focuses on the setting where the entire video is available for processing. Works such as \cite{baccouche2010action}\cite{donahue2015longterm}\cite{karpathy2014large}\cite{ng2015beyond}, incorporate temporal information in their learning process, but ultimately use the entire video for predictions. Furthermore, they target a setting where the classes are known beforehand and can be trained for. The focus of this work is a setting where the target class is unknown, and the performance is evaluated as a function of the amount of the video streamed.

\subsection{Video Concept Detection}
Concept detection in video is mainly addressed as a supervised classification task to detect objects, actions and events in videos~\cite{SnoekFNTIR09}.

briefly concept tradition in video \cite{SnoekFNTIR09}, pooling for video \cite{jiang2010trecvid,xu2015,NagelBMVC15}


\subsection{Classification without examples}
Zero-shot classification seeks to transfer the models learned on one set of classes to another related class through some intermediary knowledge source. The problem of live video retrieval is distinct from this both in being a retrieval problem, and because the nature of the input query may be radically different from the nature of the learned information. Still, the work from within the zero-shot community can be adapted to this new problem. While some zero-shot classification work relies on rigid, structured knowledge \cite{lampert2009learning}, others rely on larger linguistic corpora for knowledge transfer. Though used in zero-shot classification for narrow knowledge transfer among similar classes (e.g., types of animals, or objects), this latter approach has an open-ended nature that is well-suited for unanticipated queries. Using a sufficiently large linguistic corpus means that potential queries are restricted only by the contents of the corpus.

\cite{jain2015objects}

\minisubsection{Temporal localisation}
State-of-the-art approaches to traditional video retrieval tasks often rely on average or max pooling over the temporal axis to generate video-level feature descriptions \cite{trecvid}. In a video stream setting, only frames from the stream start to the current time are available. It is possible to adapt this pooling approach to the on-line setting of streaming by pooling in all frames from time $t=0$ to the present, but this can introduce problems. There is no guarantee that the topic will remain constant throughout the duration of a stream, especially in the case of a very long stream. For this reason, we apply temporal pooling over a limited memory. Temporally restricted pooling has been used in action detection settings, but in a different manner. \cite{oneata} uses a temporal sliding window approach with a fixed stride for the task of action detection, however this approach is a means of segmenting a video to identify when events took place in a video, rather than segmenting a live video to identify events currently taking place in it.

Recently, some work \cite{geest2016online} has tackled evaluation of online action prediction by using an average precision score across all frames of a video, however this differs significantly from our retrieval setting. Stream retrieval seeks to rank concurrent streams at any given time, measuring a comparison among streams, rather than measure the temporal performance within each single stream.


Works such as \cite{akata2013label} and \cite{lampert2009learning} use structured, expert-provided attribute information to perform zero-shot classification, which is not an option when maximizing target class breadth.

Several works have tackled zero-example prediction with videos. Notably, Objects2Actions \cite{jain2015objects} uses a similar approach to the one in this paper for the transfer from a battery of object classifiers to video classification. However, their task is action classification and temporal localization instead of retrieval over time, and the entire video is available for use in their setting.

Also related is the task of zero-shot event retrieval, particularly the Ad-Hoc Multimedia Event Detection task in the TRECVID benchmark. The Ad-Hoc Multimedia Event Detection task differs in several ways from our setting. The input is a long text describing an event, while we target short queries the sort that might arrive from users of a search engine. Videos within the TRECVID dataset are single-class and the classes are only event types, a very specific level of abstraction. Most crucially, however, the MED task involves processing and ranking of the entire video, and no evaluation along the temporal axis is considered.

The approach used within this paper for the transfer between classes is well established in state of the art literature \cite{norouzi2013zero}, and has been applied to many zero-example tasks such as object prediction, action prediction, scene prediction, ...



